Mather classes and conormal spaces of Schubert varieties in cominuscule spaces

Let $G/P$ be a complex cominuscule flag manifold. We prove a type independent formula for the torus equivariant Mather class of a Schubert variety in $G/P$, and for a Schubert variety pulled back via the natural projection $G/Q \to G/P$. We apply this to find formulae for the local Euler obstructions of Schubert varieties, and for the torus equivariant localizations of the conormal spaces of these Schubert varieties. We conjecture positivity properties for the local Euler obstructions and for the Schubert expansion of Mather classes. We check the conjectures in many cases, by utilizing results of Boe and Fu about the characteristic cycles of the intersection homology sheaves of Schubert varieties. We also conjecture that certain `Mather polynomials' are unimodal in general Lie type, and log concave in type A.

==> cotcomin_table-1.tex <==
\begin{figure}

\begin{tikzpicture}[scale=.4]
\draw (-1.5,0) node[anchor=east]  {$A_{n}$};
\foreach \x in {0,2,4,6,8}
\draw[thick,fill=black!70] (\x cm,0) circle (.3cm);
\draw[dotted, thick] (0.3 cm,0) -- +(1.4 cm,0);
\foreach \y in {2.3,4.3}
\draw[thick] (\y cm,0) -- +(1.4 cm,0);
\draw[dotted, thick] (6.3 cm,0) -- +(1.4 cm,0);
\draw (0,.8) node {$\scriptscriptstyle{1}$};
\draw (2,.8) node {$\scriptscriptstyle{d-1}$};
\draw (4,.8) node {$\scriptscriptstyle{d}$};
\draw (6,.8) node {$\scriptscriptstyle{d+1}$};
\draw (8,.8) node {$\scriptscriptstyle{n}$};

\draw (14,0) node[anchor=east]  {$B_n$};
\draw (25,0) node[anchor=west]  {\ };
\draw (14,-1.5) node[anchor=east]  {$\scriptstyle{n\geq 2}$};
\foreach \x in {18,20,22,24}
\draw[thick,fill=white!70] (\x cm,0) circle (.3cm);
\draw[thick,fill=black!70] (16 cm,0) circle (.3cm);
\draw[dotted,thick] (18.3 cm,0) -- +(1.4 cm,0);
\foreach \y in {16.3,20.3}
\draw[thick] (\y cm,0) -- +(1.4 cm,0);
\draw[thick] (22.3 cm, 1 mm) -- +(14 mm,0);
\draw[thick] (22.3 cm, -1 mm) -- +(14 mm,0);
\draw[thick] (22.9 cm, 3 mm) -- +(3 mm, -3 mm);
\draw[thick] (22.9 cm, -3 mm) -- +(3 mm, 3 mm);
\draw (16,.8) node {$\scriptscriptstyle{1}$};
\draw (18,.8) node {$\scriptscriptstyle{2}$};
\draw (20,.8) node {$\scriptscriptstyle{n-2}$};
\draw (22,.8) node {$\scriptscriptstyle{n-1}$};
\draw (24,.8) node {$\scriptscriptstyle{n}$};
\end{tikzpicture}

\vspace{3mm}

\begin{tikzpicture}[scale=.4]
\draw (-0.8,0) node[anchor=east]  {$C_{n}$};
\draw (-0.8,-1.3) node[anchor=east]  {$\scriptstyle{n\geq 2}$};
\foreach \x in {0.5,2.5,4.5,6.5}
\draw[thick,fill=white!70] (\x cm,0) circle (.3cm);
\draw[thick,fill=black!70] (8.5 cm,0) circle (.3cm);
\draw[thick] (0.8 cm,0) -- +(1.4 cm,0);
\draw[dotted,thick] (2.8 cm,0) -- +(1.4 cm,0);
\draw[thick] (4.8 cm,0) -- +(1.4 cm,0);
\draw[thick] (6.8 cm, .1 cm) -- +(1.4 cm,0);
\draw[thick] (6.8 cm, -.1 cm) -- +(1.4 cm,0);
\draw[thick] (7.4 cm, 0 cm) -- +(.3 cm, .3 cm);
\draw[thick] (7.4 cm, 0 cm) -- +(.3 cm, -.3 cm);
\draw (0.5,.8) node {$\scriptscriptstyle{1}$};
\draw (2.5,.8) node {$\scriptscriptstyle{2}$};
\draw (4.5,.8) node {$\scriptscriptstyle{n-2}$};
\draw (6.5,.8) node {$\scriptscriptstyle{n-1}$};
\draw (8.5,.8) node {$\scriptscriptstyle{n}$};

\draw (14,0) node[anchor=east]  {$D_{n}$};
\draw (14,-1.3) node[anchor=east]  {$\scriptstyle{n\geq 4}$};
\foreach \x in {17,19,21,23}
\draw[thick,fill=white!70] (\x cm,0) circle (.3cm);
\draw[thick,fill=black!70] (15 cm,0) circle (.3cm);
\draw[xshift=23 cm,thick,fill=black!70] (30: 17 mm) circle (.3cm);
\draw[xshift=23 cm,thick,fill=black!70] (-30: 17 mm) circle (.3cm);
\draw[dotted,thick] (19.3 cm,0) -- +(1.4 cm,0);
\foreach \y in {15.3, 17.3, 21.3}
\draw[thick] (\y cm,0) -- +(1.4 cm,0);
\draw[xshift=23 cm,thick] (30: 3 mm) -- (30: 14 mm);
\draw[xshift=23 cm,thick] (-30: 3 mm) -- (-30: 14 mm);
\draw (15,.8) node {$\scriptscriptstyle{1}$};
\draw (17,.8) node {$\scriptscriptstyle{2}$};
\draw (19,.8) node {$\scriptscriptstyle{3}$};
\draw (21,.8) node {$\scriptscriptstyle{n-3}$};
\draw (23,.8) node {$\scriptscriptstyle{n-2}$};
\draw (24.45,1.6) node {$\scriptscriptstyle{n-1}$};
\draw (24.45,-.2) node {$\scriptscriptstyle{n}$};

\end{tikzpicture}


\vspace{1mm}


\begin{tikzpicture}[scale=.4]
\draw (-2.4,0) node[anchor=east]  {$E_{6}$};
\foreach \x in {1,3,5}
\draw[thick,fill=white!70] (\x cm,0) circle (.3cm);
\draw[thick,fill=white!70] (3 cm, 2 cm) circle (.3cm);
\foreach \x in {-1,7}
\draw[thick,fill=black!70] (\x cm,0) circle (.3cm);
\foreach \y in {-0.7, 1.3, 3.3, 5.3}
\draw[thick] (\y cm,0) -- +(1.4 cm,0);
\draw[thick] (3 cm,.3 cm) -- +(0,1.4 cm);
\draw (-1,.8) node {$\scriptscriptstyle{1}$};
\draw (1,.8) node {$\scriptscriptstyle{3}$};
\draw (3.5,.8) node {$\scriptscriptstyle{4}$};
\draw (5,.8) node {$\scriptscriptstyle{5}$};
\draw (7,.8) node {$\scriptscriptstyle{6}$};
\draw (3.5,2.8) node {$\scriptscriptstyle{2}$};

\draw (12,0) node[anchor=east]  {$E_{7}$};
\foreach \x in {13,15,17,19,21}
\draw[thick,fill=white!70] (\x cm,0) circle (.3cm);
\draw[thick,fill=white!70] (17 cm, 2 cm) circle (.3cm);
\draw[thick,fill=black!70] (23 cm,0) circle (.3cm);
\foreach \y in {13.3, 15.3, 17.3, 19.3, 21.3}
\draw[thick] (\y cm,0) -- +(1.4 cm,0);
\draw[thick] (17 cm,.3 cm) -- +(0,1.4 cm);
\draw (13,.8) node {$\scriptscriptstyle{1}$};
\draw (15,.8) node {$\scriptscriptstyle{3}$};
\draw (17.5,.8) node {$\scriptscriptstyle{4}$};
\draw (19,.8) node {$\scriptscriptstyle{5}$};
\draw (21,.8) node {$\scriptscriptstyle{6}$};
\draw (23,.8) node {$\scriptscriptstyle{7}$};
\draw (17.5,2.8) node {$\scriptscriptstyle{2}$};

\end{tikzpicture}

\vspace{4mm} 
\caption{(see \cite{bourbaki}) Finite type Dynkin diagrams with cominuscule simple roots marked in black (left column).}
\label{TBL:comin}
\end{figure}


==> data/cMaGr47.tex <==
\begin{table}
\centering
\captionsetup[subfloat]{labelformat=empty}
\subfloat[][]{
\noindent\makebox[\textwidth]{%This line of code copied from https://tex.stackexchange.com/questions/4926/table-will-not-center-and-it-is-spilling-off-the-right-side-of-the-page. See the third and fifth answer in particular.
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
&4&41&42&411&43&421&44&431&422&441&432&442&433&443&444\\\hline
()&5&10&15&15&20&30&15&40&30&30&60&45&40&60&35\\
1&10&24&42&42&64&92&60&140&108&130&228&210&190&300&210\\
2&10&26&51&48&88&117&105&203&153&240&351&411&360&624&525\\
11&0&10&29&34&56&89&65&163&141&180&315&341&330&544&455\\
3&5&14&30&27&58&71&90&139&99&215&251&387&305&621&630\\
21&0&10&36&36&82&119&120&258&216&360&541&738&690&1266&1260\\
111&0&0&0&10&0&29&0&56&66&65&155&185&205&351&350\\
31&0&5&19&19&49&67&91&166&128&297&369&652&547&1193&1407\\
22&0&0&10&0&36&36&67&121&97&214&300&502&483&968&1141\\
211&0&0&0&10&0&36&0&82&94&120&252&375&397&768&896\\
32&0&0&5&0&24&19&58&86&54&199&229&505&434&1056&1470\\
311&0&0&0&5&0&19&0&49&51&91&157&298&278&645&868\\
221&0&0&0&0&0&10&0&36&46&67&157&281&318&678&938\\
33&0&0&0&0&5&0&18&19&0&65&54&174&136&408&680\\
321&0&0&0&0&0&5&0&24&24&58&110&257&257&672&1076\\
222&0&0&0&0&0&0&0&0&10&0&36&67&100&228&376\\
331&0&0&0&0&0&0&0&5&0&18&24&83&78&257&497\\
322&0&0&0&0&0&0&0&0&5&0&24&58&80&224&427\\
332&0&0&0&0&0&0&0&0&0&0&5&18&29&101&238\\
333&0&0&0&0&0&0&0&0&0&0&0&0&5&18&56\\
4&1&3&7&6&15&17&31&37&25&77&69&145&90&245&301\\
41&0&1&4&4&11&15&26&40&30&93&93&218&146&423&588\\
42&0&0&1&0&5&4&16&19&12&59&54&163&108&368&604\\
411&0&0&0&1&0&4&0&11&11&26&36&88&66&198&302\\
43&0&0&0&0&1&0&6&4&0&23&12&66&32&168&336\\
421&0&0&0&0&0&1&0&5&5&16&24&75&58&207&378\\
44&0&0&0&0&0&0&1&0&0&4&0&12&0&32&80\\
431&0&0&0&0&0&0&0&1&0&6&5&29&17&95&215\\
422&0&0&0&0&0&0&0&0&1&0&5&16&17&65&141\\
441&0&0&0&0&0&0&0&0&0&1&0&5&0&17&49\\
432&0&0&0&0&0&0&0&0&0&0&1&6&6&35&98\\
442&0&0&0&0&0&0&0&0&0&0&0&1&0&6&23\\
433&0&0&0&0&0&0&0&0&0&0&0&0&1&6&24\\
443&0&0&0&0&0&0&0&0&0&0&0&0&0&1&7\\
444&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1\\
\hline
\end{tabular}
}
}
\caption{ Chern-Mather classes for $\Gr(4,7)$.  }
\label{TBL:Gr47}
\end{table}



==> data/cMaLG36.tex <==
\begin{table}
\centering
\captionsetup[subfloat]{labelformat=empty}
\subfloat[][]{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
    & () & 1 & 2 & 3 & 21 & 31 & 32 & 321\\ \hline
()  & 1  & 2 & 2 & 4 & 4  & 8  & 4  & 8\\
1   & 0  & 1 & 4 & 9 & 8  & 20 & 18 & 36\\
2   & 0  & 0 & 1 & 5 & 3  & 14 & 23 & 46\\
3   & 0  & 0 & 0 & 1 & 0  & 3  & 7  & 15\\
21  & 0  & 0 & 0 & 0 & 1  & 5  & 18 & 37\\
31  & 0  & 0 & 0 & 0 & 0  & 1  & 6  & 15\\
32  & 0  & 0 & 0 & 0 & 0  & 0  & 1  & 4\\
321 & 0  & 0 & 0 & 0 & 0  & 0  & 0  & 1\\
\hline
\end{tabular}
}
\caption{
Chern-Mather classes for $LGr(3,6)$.
The Schubert varieties are indexed by certain partitions, see ADDREF.
The expansion of the Chern-Mather class of a Schubert variety 
in terms of ordinary Schubert classes 
is given in the column indexed by the corresponding partition. 
}
\end{table}

